On Process Awareness in Detecting Multi-stage Cyberattacks in Smart Grids

This study delves into the role of process awareness in enhancing intrusion detection within Smart Grids, considering the increasing fusion of ICT in power systems and the associated emerging threats. The research harnesses a co-simulation environment, encapsulating IT, OT, and ET layers, to model multi-stage cyberattacks and evaluate machine learning-based IDS strategies. The key observation is that process-aware IDS demonstrate superior detection capabilities, especially in scenarios closely tied to operational processes, as opposed to IT-only IDS. This improvement is notable in distinguishing complex cyber threats from regular IT activities. The findings underscore the significance of further developing sophisticated IDS benchmarks and digital twin datasets in Smart Grid environments, paving the way for more resilient cybersecurity infrastructures.

==> chapter1_old.tex <==
\section{Introduction}
The transformation of traditional power grids into \acp{sg} has led to significant changes in \ac{ict} infrastructure. Earlier, \acp{sg} were characterized by isolated and proprietary components, limiting external third-party integration. However, the growing integration of \ac{ict} in these grids has led to enhanced connectivity, which, in turn, has introduced new cybersecurity vulnerabilities, notably cyberattacks~\cite{pan2015developing}.

A crucial element in addressing these cybersecurity challenges is the detection process. Commonly recommended solutions such as \acp{ids} often depend heavily on \ac{ict} data and may overlook essential underlying processes and domain-specific knowledge critical for identifying new threats and validating alerts. This is where the concept of 'process awareness' in \acp{ids} becomes critical, particularly in \acp{sg} with unique domain attributes. Process-aware \acp{ids} leverage domain-specific knowledge to pinpoint abnormal behaviors in the system accurately. Given the predictable nature of grid traffic and standard configurations, process awareness is increasingly recognized as a key factor for effective \acp{ids} in \acp{sg}. These systems have become essential in identifying unusual activities and cybersecurity threats~\cite{shun2008network}. An \ac{ids} is typically a software tool designed to detect malicious activities within a network or system~\cite{wagle2021utilizing}.

Despite advancements, current \acp{ids} still encounter challenges like enhancing detection accuracy, minimizing false positives, and identifying unknown attacks. Machine learning has become a pivotal area of research to overcome these challenges due to its potential for high accuracy and the ability to generalize in detecting novel attacks~\cite{liu2019machine}. However, these machine learning methods often grapple with high rates of false positives and a lack of clarity in their alert mechanisms~\cite{samrin2017review, kus2022false}.

An effective anomaly detection system, offering high precision and clear, explainable alerts, is needed to reduce both the effort and expertise required in processing a large volume of alerts and to improve the accuracy and speed of situation analysis and response. This necessitates a detection approach that is both reliable and transparent in its decision-making process.

In environments like \ac{ics} and \acp{sg}, it's crucial to detect anomalies in process data. Machine learning-driven \acp{ids} often utilize techniques like allowlisting, which identifies deviations from normal system operations, and blocklisting, focusing on predefined abnormal behaviors. These anomalies can be indicative of various issues, such as cyberattacks, system errors, or configuration mistakes, manifesting in different ways, including protocol anomalies or communication disruptions.

Consequently, the challenges that we address in this paper are:
\begin{itemize}
\item Identifying and effectively leveraging significant domain knowledge inherent to electrical grid operations, which is crucial for detecting cyber threats and enhancing the capabilities of \ac{ids}.
\item Integrating relevant indicators from diverse domains such as \ac{it}, \ac{ot}, and \ac{et}. This includes understanding the attributes of attack indicators that are inherent to the respective \ac{ics} layers.
\item Understanding the impact of different domains on attack detection, particularly process-aware detection techniques for the \ac{sg}.
\end{itemize}

In this paper, we aim to explore the effectiveness of process-awareness in identifying complex, multi-stage cyberattacks in \acp{sg}. We combine comprehensive \ac{sg} knowledge with traditional \ac{ict} intrusion detection methods to enhance overall grid security. A detailed simulation environment is utilized, reflecting all aspects of \ac{sg} operations, including their \ac{it}, \ac{ot}, and \ac{et} components. Our research employs a layered approach, wherein sensors monitor the grid for anomalies and relay this information to a central system that integrates domain knowledge for enhanced process awareness. This system not only analyzes \ac{ict} traffic anomalies but also scrutinizes process data from \ac{scada} systems. By correlating these different types of data, we can form a complete picture of potential cyber incidents. Thus, our investigation delves into how process-awareness can improve the quality of detection, contrasting various cyberattack scenarios and analyzing the resulting indicators. The findings, with a particular focus on \ac{scada} anomalies, provide insights into the advantages of integrating different types of data for more effective detection. The overarching goal is an in-depth exploration of process-aware detection methods in a simulated \ac{sg} environment, striving to achieve a more comprehensive understanding and enhancement of grid security.

Our contributions are therefore:
\begin{itemize}
\item Investigating the effectiveness of process-awareness in identifying complex, multi-stage cyberattack within \acp{sg}, and combining \ac{sg} knowledge with traditional \ac{ict} intrusion detection methods.
\item Employing a comprehensive simulation environment that reflects all aspects of \ac{sg} operations, encompassing \ac{it}, \ac{ot}, and \ac{et} components, to monitor and analyze grid anomalies and \ac{ict} traffic, thus enhancing grid security.
\item Implementing a layered approach with sensors and central systems that integrate domain knowledge for process awareness. This approach focuses on \ac{scada} system anomalies and correlates different data types for an in-depth exploration of effective detection methods in a simulated \ac{sg} environment.
\end{itemize}

The paper is structured as follows: In Section~\ref{background:ov}, we provide an analysis of process-aware \ac{ids} in \ac{ics}, forming the foundation of this work. We then describe our investigation framework for addressing the established research subject in Section~\ref{sec:methodology}. The experimental findings and discussion are presented in Section~\ref{sec:result}. We conclude this paper with a summarization of the key findings and a future outlook in Section~\ref{sec:conclusion}.


==> chapter2_old.tex <==
\section{Process Awareness in IDS}\label{background:ov}
In Section~\ref{background:ids}, we establish our understanding of \ac{ids}, its function in the context of anomaly detection, and its main features in terms of explainability, while in Section~\ref{background:processawanress}, the characteristics of process awareness are elaborated. Section~\ref{background:purdue} builds upon the established Purdue Model for \ac{ics}, and in Section~\ref{background:machinelaerningids}, we analyze the machine learning-based stacked meta-learner for anomaly detection. We also present related work in the context of machine learning-based \ac{ids} and the investigation of process-aware \ac{ids} in Section~\ref{background:related_work}.

\begin{figure}\textbf{}
    \centering
    \includegraphics[width=\columnwidth]{figures/ICS_Architektur.pdf}
    \caption{Illustration of \ac{ids} integration into \ac{sg} industrial control architecture and anomalies in the environment}
    \label{fig:ids_in_ics}
\end{figure}

\subsection{Intrusion Detection Systems}\label{background:ids}
An \ac{ids} is a critical security solution that can be either software or hardware-based, designed to monitor and analyze network or system activities to detect potential cyber threats such as unauthorized access, misuse, or disruption. \acp{ids} can be implemented in various forms, including on individual devices or across a network, and they are capable of monitoring a wide range of data types, including device logs, network traffic, and process data, to identify suspicious or malicious activities.

\acp{ids} are often categorized based on the source of their data into network-based and host-based systems. Host-based \acp{ids} operate directly on devices, scanning for malicious behaviors like file modifications~\cite{hu2009simple}, while network-based \acp{ids} analyze network traffic, such as packets or flow-data, to detect malicious activities~\cite{ring2019survey}. This distinction is particularly relevant in \ac{ics} environments, such as \ac{sg}, where process-aware \acp{ids} are critical. These systems can recognize and analyze process data, including measurements or control commands, and detect anomalies at the process level.

Machine learning-based \acp{ids} employ sophisticated methods for detecting anomalies. Two primary approaches used are allowlisting and blocklisting. Allowlisting focuses on identifying deviations from normal system behavior learned by the model, whereas blocklisting identifies known abnormal behaviors represented in the trained model. In both approaches, anomalies may indicate cyberattacks, system malfunctions, or misconfigurations, manifesting as protocol errors, missing messages, communication aborts, and more. These methods leverage network structure, system discovery, and connection behavior to validate the legitimacy of devices, protocols, and communication patterns.

An essential aspect of machine learning-based \acp{ids} is explainability, which refers to the capability to qualitatively understand the relationship between model input and prediction in a user-friendly manner~\cite{islam2020towards}. Explainability can be provided through local explanations, which elucidate a model's behavior on a specific input instance, or global explanations, which offer insights into the inner workings of a model's behavior. These methods can be either model-agnostic or model-specific, playing a crucial role in verifying results and maintaining confidence in the system's predictions.

\subsection{Process Awarness}\label{background:processawanress}
Process-awareness in intrusion detection refers to the ability to utilize domain-specific knowledge for detecting anomalies. For instance, from known and confirmed communication patterns learned through the model within network-based \ac{ids}, deviating communication and behavior patterns are detected as an anomaly (cf. Figure~\ref{fig:ids_in_ics}). 
In particular, for deterministic and highly automated \ac{ics} such as the \ac{sg}, these can be the following attributes: unknown devices, new connections, attacks on other segments, or altered function of the communication.
In this context, anomalies are not necessarily due to cyberattacks but also to fault conditions indicating plant or network malfunctions, manifested for example by protocol errors, missing or delayed cyclic messages, or messages in the wrong order in connection-oriented protocols.
%In this context, anomalies are not necessarily due to cyberattacks but also to fault conditions indicating plant or network malfunctions, manifested for example by protocol errors, missing or delayed cyclic messages, communication aborts, changed packet round-trip time, packet flow control malfunction, missing protocol flows, or messages in the wrong order in connection-oriented protocols.
Within the network-based interactions between different devices in the system's industrial control architectures, the traffic contains special information that can be leveraged for interactive network detection.
For instance, the learned network structure, system discovery, and connection behavior can provide essential details about the legitimacy of the system's physical and logical components, such as IP and MAC addresses, communication traffic with other components, protocols and functions used over time, and more.
%For instance, the learned network structure, system discovery, and connection behavior can provide essential details about the legitimacy of the system's physical and logical components, such as IP and MAC addresses, vendor information, connections and data flows between components, communication traffic with other components, protocols and functions used over time, operating system or firmware versions, and more.

Detection of physics-related data in the form of process data within traffic containing industrial protocol data is also part of anomaly detection, which includes plausibility checks of observed system-related information such as measurements or control commands.

Anomalies in \acp{ics}, such as \acp{sg}, can include any deviation from the normal and expected communication patterns within the network.
This can include unknown devices, new connections, attacks on different segments, and altered communication functions.
%Anomalies can also be caused by fault conditions, such as protocol errors, missing or delayed messages, communication aborts, and changes in packet flow.
By leveraging the special information present in the traffic, it is possible to detect such anomalies and assess the legitimacy of the system's physical and logical components.
%By leveraging the special information present in the traffic, such as system structure, connections and data flows, and device information, it is possible to detect such anomalies and assess the legitimacy of the system's physical and logical components.
%Detection of process data in the form of measurements or control commands is also an important aspect of anomaly detection.

\subsection{Purdue Model}\label{background:purdue}
The Purdue Model, a key component of \ac{pera}~\cite{williams1996overview}, serves as a vital framework for understanding the various layers and components of \ac{ics} networks, and is instrumental in selecting appropriate datasets for benchmarking purposes. This model delineates the \ac{ics} architecture into two primary zones: the \ac{ot} zone, consisting of physical equipment and operational process control systems, and the \ac{it} zone, which includes systems for data management and communication. Additionally, a \ac{dmz} is established between the \ac{it} and \ac{ot} zones to regulate access. The model divides the \ac{ics} architecture into six distinct levels:
The hierarchical structure of \ac{ics} is delineated through six distinct levels. At the base, Level 0 contains the physical hardware such as transformers and circuit-breakers. Level 1 incorporates controllers like \acp{plc} and \acp{rtu} that manage the Level 0 devices. Ascending to Level 2, we find the supervisory systems, including \ac{hmi} and \ac{scada} software, which oversee \ac{ics} operations. Level 3 is dedicated to managing production workflows, while Level 4 extends to systems handling logistics and data storage. The top tier, Level 5, encompasses the enterprise network, integrating \ac{ics} data for strategic business decision-making.

Utilizing the Purdue model (refer to Section~\ref{background:purdue}), it is essential to select datasets that accurately reflect real-world attack scenarios and correspond to specific levels of \ac{ics}. This approach significantly enhances the relevance of evaluating \acp{ids} within \ac{ics} settings. For example, datasets that address anomalies at Levels 0 to 2 are crucial, as they focus on physical components and control systems. Similarly, datasets covering intrusion and attack scenarios at Levels 3 and 4 are also vital. In addition, datasets specifically designed for anomalies at Levels 4 and 5, which are concerned with managing logistics and communications, are imperative. These datasets collectively offer a comprehensive range of anomalies, thereby facilitating the effective evaluation of \acp{ids} in their ability to detect and classify various network-based threats in \ac{ics} environments.

For a thorough evaluation of process-aware \acp{ids} in \ac{ics}, including \ac{sg}, it is essential to have a simulation environment that includes a diverse range of anomalies representative of real-world attack types. Such an environment ensures that the \acp{ids} are rigorously tested against a wide variety of relevant attack scenarios, thereby enhancing their robustness and practical applicability in \ac{ics} contexts. Emphasis is placed on the utilization of structured, labeled, and network-based datasets for this evaluation. Furthermore, integrating explainable methods into \acp{ids} is crucial for providing clear insights into their decision-making processes. This integration not only builds trust in these systems but also plays a significant role in effectively reducing the occurrence and impact of false positives.

\subsection{Machine Learning based IDS}\label{background:machinelaerningids}
For the machine learning based \ac{ids} several vital preprocessing steps are required, such as data transformations, cleaning, reduction, discretization, and re-labeling. Although feature construction and dataset creation are excluded due to their dependency on specific protocols and dataset features, other preprocessing methods are recommended to be flexible and optional in the evaluation process~\cite{davis2011data}.

Ensemble learning, particularly stacking methods, is increasingly used to enhance classification performance in \acp{ids}. This approach involves combining multiple learning algorithms, to synthesize their predictions. The framework allows for the analysis of various stacking algorithms and the customization of base classifiers.
%Ensemble learning, particularly stacking methods, is increasingly used to enhance classification performance in \acp{ids}. This approach involves combining multiple learning algorithms, referred to as first-level models, and using another model, the second-level model, to synthesize their predictions. The framework allows for the analysis of various stacking algorithms and the customization of base classifiers.

Evaluation metrics for \acp{ids} are application-specific, with high detection accuracy, runtime efficiency, and explainability being key criteria. The robustness of \acp{ids} is essential for improved detection accuracy, and the diversity in ensemble methods is a critical aspect to be assessed~\cite{liu2019machine, zhou2012ensemble}. Binary classification is selected as the primary evaluation task, utilizing multiple datasets and incorporating statistical tests and confidence intervals to ensure reproducibility and control of randomization in the model evaluation.

Moreover, the increasing complexity of machine learning methods in \acp{ids} necessitates the inclusion of explainability to maintain confidence in the results and verify their accuracy. Explainability in machine learning-based \acp{ids} not only bolsters confidence in generated alerts but also aids in post-incident analysis, potentially identifying root causes and minimizing false positives. The formal definitions of explainability emphasize the importance of providing a qualitative understanding of the relationship between model input and prediction in a user-friendly manner~\cite{islam2020towards}. Local explanations focus on individual input instances~\cite{lundberg2020local}, while global explanations aim to elucidate the model's overall behavior~\cite{covert2020understanding}.% Methods of explainability can be divided into model-agnostic, applicable to any model, and model-specific, tailored to a particular type of model.

\subsection{Related Work}\label{background:related_work}
The research landscape has been actively exploring the development of benchmark environments to evaluate the performance of various machine learning algorithms in detecting anomalies and intrusions within \ac{ics}. Approaches like the Penn Machine Learning Benchmark~\cite{olson2017pmlb} and the Scientific Machine Learning Benchmark suite~\cite{thiyagalingam2022scientific} provide vital resources for testing and comparing algorithm performance. Researchers have also emphasized the creation of datasets from real \ac{ics} environments, such as the Cyber-kit datasets~\cite{mubarak2021ics} and the Numenta anomaly benchmark~\cite{lavin2015evaluating}, to evaluate unsupervised anomaly detection techniques or \acp{ids} in \ac{ics}. Specific focus has been given to datasets related to \acp{sg} to assess the performance of machine learning algorithms in detecting anomalies in these systems~\cite{bernieri2019evaluation, liyakkathali2020validating, mohammadpourfard2019benchmark}. However, there exists a need for more specialized and comprehensive approaches, particularly in considering the unique characteristics and constraints of \ac{ics} and \acp{sg}, such as explainability of algorithms and statistical confidence of findings~\cite{japkowicz2006question, tufan2021anomaly}.

In addition, research works have investigated process-aware \acp{ids} in \ac{ics}, focusing on evaluating the criticality of \ac{ics} devices and identifying potential adversary traces~\cite{15_cook2017industrial, 16_escudero2018process}. Advanced approaches include the replication of program states in digital twins~\cite{9_eckhart2018specification}, cyber-attack classification~\cite{18_mohan2020distributed}, and modeling \ac{ics}/\ac{scada} communication using probabilistic automata~\cite{19_matouvsek2021efficient, 20_almseidin2019fuzzy}. Anomaly detection methods for \ac{iec104} have also been explored using multivariate access control and outlier detection approaches~\cite{grammatikis2020anomaly, burgetova2021anomaly, anwar2021comparison}. However, these proposed approaches require additional analytical resources for their functionality, such as infrastructure specifications, attack target understanding, statistical data, or technical specifications~\cite{scheben2017status, dang2021improving, holzinger2020measuring}. Process awareness in \ac{ids} has not been systematically investigated, particularly in terms of its specific contribution to the general detection of cyberattacks and the added value it provides across different domain spaces of \ac{ics}.

This paper aims to delve into the realm of process awareness in \ac{ids}, particularly focusing on how domain knowledge from the operation of electrical grids can be leveraged to enhance these systems. A key aspect of our investigation is the identification of significant domain knowledge inherent to grid operation that could be crucial for detecting cyberattacks. This includes an in-depth analysis of the plausibility of process data, a critical factor in discerning legitimate operations from potential security breaches. We also explore the integration of relevant indicators from diverse domains, specifically \ac{it}, \ac{ot}, and \ac{et}. This involves identifying domain-specific attributes of the indicators with regard to detecting multi-stage cyber attacks impacting several domains in the \ac{ics} layer hierarchy.



==> chapter3_old.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{figures/plantuml_overview.pdf}
    \caption{Overview of the class diagrams of the co-simulation for the investigation of process-aware \ac{ids}}
    \label{component_diag}
\end{figure}

\section{Investigation Framework}\label{sec:methodology}
In this section, we present the investigation framework developed to investigate process awareness in \ac{ids}. In Section~\ref{sec:methodology_overview}, we provide a general overview of the framework, while Section~\ref{subsec:methodology-req} is dedicated to performing the requirement analysis for the approach. In Section~\ref{subsec:methodology-investigation}, we introduce the investigation environment and the corresponding attack, as well as the \ac{ids} implementation, which includes the generation (cf. Section~\ref{subsec:mutlistage_implementation}) and detection of different anomalies (cf. Section~\ref{subsec:methodology-ids}).

\subsection{Overview}\label{sec:methodology_overview}
Our paper presents a comprehensive exploration of enhancing \ac{ids} with process awareness, focusing particularly on the application within electrical grid operations. It underscores the integration of domain knowledge from both \ac{it} and \ac{ot} sectors, which is essential for nuanced detection of cyber threats in \ac{sg}. The heart of our research lies in the analysis of process data within these grids, aiming to distinguish authentic operational activities from potential cybersecurity threats. This involves a deep dive into correlating and combining indicators across \ac{it} and \ac{ot} domains to enhance the accuracy and breadth of \ac{ids}. Moreover, we emphasize the development of criteria to differentiate between normal and anomalous process data in complex situations, where system faults may not necessarily indicate cyberattacks. The Figure~\ref{component_diag}  serves as a visual representation of the investigation framework. It showcases the dynamic interplay between various elements such as energy technologies and operational technologies within a co-simulation environment, encapsulating the complex interactions and dependencies inherent in electrical grids. The framework depicted in the diagram is instrumental for our research, as it provides a structured approach to analyze the plausibility of process data and develop criteria to distinguish between legitimate and illegitimate data traffic. This visual representation not only underscores the complexity of the task at hand but also conveys how our approach aims to bolster the effectiveness and proactivity of \ac{ids} in maintaining grid security under varying infrastructural and managerial conditions.

\subsection{Requirement Analysis}\label{subsec:methodology-req}
Reproducibility is the capacity to reproduce the exact outcomes presented by a study's author~\cite{tatman2018practical,uetz2021reproducible}.
To attain a high level of reproducibility in studies, essential components include datasets, data preprocessing, model training, model evaluation, and the software \& hardware environment of the model~\cite{olorisade2017reproducibility, thiyagalingam2022scientific}.

The integrity of datasets is vital for appraising machine learning-based \acp{ids} within \acp{ics}, especially in \ac{sg}.
For real-world relevance, datasets should be chosen based on the Purdue Model, which offers insights into an \ac{ics}'s layers~\cite{williams1996overview}.
Datasets must be domain-specific, balanced, labeled, and confined to network-based data~\cite{demvsar2006statistical}.

Crucial preprocessing steps for network-based \acp{ids} encompass data transformations, cleaning, reduction, discretization, and re-labeling.
This work emphasizes the applicability of multiple preprocessing methods without one impeding another~\cite{davis2011data}.

Combining multiple learning algorithms, ensemble models (or stacking) are paramount.
Metrics for evaluation should cater to detection accuracy, runtime efficiency, explainability, robustness, and diversity~\cite{zhou2012ensemble, liu2019machine}.
Binary classification is preferred, and statistical tests ensure result generalizability~\cite{witten2002data}.

Complete study documentation ensures reproducibility, necessitating information on datasets, preprocessing, model training, and evaluation methods, plus the hardware and software environment.
The scope of this work revolves around processs-aware anomaly-based network \acp{ids} for \acp{sg}, emphasizing machine learning and binary classification.

The Purdue model forms a backbone for representing the \ac{sg} infrastructure, especially the \ac{scada} application~\cite{williams1996overview}.
In replicating real-world threats and their effects, a \ac{cps} co-simulation approach is proposed, leveraging both physical and cyber aspects.
The challenge is finding a balance between physically operated testbeds and complex simulations.
A hybrid strategy, employing emulation and selective simulation, offers an optimal compromise.

\subsection{Investigation Environment}\label{subsec:methodology-investigation}
Our work revolves around the development of a comprehensive co-simulation framework tailored for energy information networks.
At its core, this methodology amalgamates a variety of individual simulators and models.
These integrated models cater to different aspects of energy and process networks, creating a holistic understanding of the system.

In our work, we categorize the \ac{dso} infrastructure into three principal domains, each with distinct roles and components. The \ac{et} domain includes essential elements like switches and transformers, which are crucial for efficient electricity distribution. The \ac{ot} domain features \acp{ied} that link primary units to the OT network, supporting crucial functions such as control and measurement. These \acp{ied} primarily communicate data to the \ac{scada} system using protocols like \ac{iec104}. Lastly, the \ac{it} domain covers systems that facilitate remote maintenance and external communications. Within this domain, the \ac{scada} system emerges as a critical element, bridging the \ac{ot} network and office network through a \ac{dmz}.

A significant focus of the simulation is on the component-based, modular simulation of distribution network infrastructures, accommodating networks with diverse characteristics and sizes. This allows for extensive and varied investigative scenarios that require a cohesive modeling approach to the entire system. The design and utility of the co-simulation are predominantly defined by the need for a realistic depiction of the individual components across \ac{it} and \ac{ot} domains and their communication behaviors. This aspect is crucial for systematically representing \ac{ict} failures and cyberattacks, whether targeting individual components or groups within the network, thus making the co-simulation a versatile and essential tool in understanding and enhancing the resilience of energy information networks.

The co-simulation process in our study is structured into three critical stages. Firstly, the Deployment phase involves the creation of network topology, setting up model parameters, and establishing the co-simulation environment. Secondly, the Execution phase entails initiating the simulation, ensuring synchronized and real-time data transfer between the components. Finally, the Evaluation phase focuses on analyzing the results post-simulation. This includes detailed visualization and extensive reporting, with a particular emphasis on understanding the impacts of cyberattacks on the power supply system.

Additionally, the co-simulation framework utilizes the Mosaik framework for central initialization, scheduling, and data exchange among the simulators~\cite{schutte2011mosaik}. Mosaik offers open interfaces, facilitating the development of simulation scenarios based on the graph-based model and enabling the connection of additional simulators. This setup allows for large-scale scenario simulations and seamless integration of real-time labs and software-in-the-loop systems into the co-simulation environment.

The \ac{ict} communication network emulation in the co-simulation, utilizing "rettij," focuses on creating a realistic representation of process networks alongside energy networks~\cite{niehaus2022modern}. "rettij" is designed to seamlessly integrate into co-simulation environments, particularly with mosaik, a co-simulation framework. This integration facilitates the realistic emulation of \ac{ict}  networks, using real network stacks and standard Linux tools to accurately represent network components like switches and routers. The simulator supports the creation of complex network topologies in a user-friendly YAML format, and its architecture allows for distributed, scalable simulations, making it a versatile tool for testing scenarios including normal operations and \ac{it} attack simulations in energy information networks.

For modeling multifaceted attack scenarios, we utilize the MITRE ATT\&CK Framework.
This framework classifies and structures attack modalities, tactics, and patterns, deriving insights from real-world attack occurrences.
While there are tracking limitations, the data is instrumental in developing an attack catalog.

The process of cyberattack in our simulation encompasses multiple stages, each with a distinct objective. It begins with the Initial Access phase, where techniques like spear-phishing are simulated to represent user interaction. The next phase, Execution, involves the attacker's steps to execute malicious code. This is followed by Privilege Escalation, where the attacker aims to gain higher access levels within the system. In the Credential Access phase, the focus is on obtaining sensitive user data. Lateral Movement comes next, spreading the attack across networked devices. The Collection phase involves gathering data about the attack target, followed by establishing a network for communication in the Command and Control phase. The final phase, Impact, marks the culmination of the attack, potentially leading to data manipulation, disruption, or destruction.

Implementing co-simulation in energy information networks necessitates merging domain-specific models and simulation settings.
This inclusive approach aids in identifying and addressing vulnerabilities, enhancing the security stature of energy information networks.

Our meticulously designed co-simulation provides a robust platform to scrutinize energy information networks.
By focusing on genuine scenarios and exhaustive vulnerability evaluations, it offers precious insights into potential cyber threats and their countermeasures.


\subsection{Multistage Attack Implementation}\label{subsec:mutlistage_implementation}
The implementation of the right multistage attacks is depicted in this section. In order to provide a best fitting coverage over the given main domains \ac{et}, \ac{ot}, and \ac{it}, the following attacks have been chosen. Note, that these attacks consist of sufficient attacks, which are required for the multistage attacks and are therefore re-used over multiple multistage attacks.

In our simulation, the multistage attacks are premised on having already gained network access. We introduce an additional node representing the attacker, equipped with various adversarial tools. This setup presumes the attacker's prolonged surveillance of the network, granting them insights into \acp{rtu}, \acp{mtu}, and switch configurations.

\ac{arp} Spoofing/Poisoning is a critical technique in our simulation. Utilizing the ARP protocol, which resolves physical addresses from network addresses, the attacker crafts custom \ac{arp}  packets to poison victims' \ac{arp} caches. This effectively masks malicious activities under legitimate IP addresses.

\ac{mitm} attacks follow, leveraging \ac{arp} poisoning to reroute specific device traffic through the attacker, enabling them to sniff and alter communication packets.

Additionally, network connection enumeration is employed, using techniques like subnet address scanning and port scanning to identify vulnerable points within the network infrastructure. These steps collectively constitute the foundational strategies of our simulated multistage cyberattacks.

For the multi-stage attack we focus on several key strategies. First, the \ac{dos} attack is designed to disrupt the \acs{mtu} in a network with 26 \acs{rtu}. This attack employs a \acs{tcp} 3-way handshake to achieve maximum impact.

The \ac{iec104} Value Modification attack is executed after establishing a \acs{mitm} position. It involves intercepting and altering local \ac{iec104} protocol traffic, either randomly or with precision to target specific system commands.

Lastly, the Replay Attack strategy captures non-malicious traffic between the \acs{mtu} and \acp{rtu}, later replaying altered packets to avoid detection of malicious activities. This attack is particularly subtle as it mimics normal traffic patterns, masking the attacker's interventions.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{figures/cosim_structure.pdf}
    \caption{Overview of the cigre-based scenario simulated in the co-simulation for the study: a) the co-simulation architecture and the components involved, b) the infrastructure model of the scenario and c) the specific network model for the case}
    \label{fig:scenario_overview}
\end{figure}

\subsection{IDS Implementation}\label{subsec:methodology-ids}
This section details the classifier utilized in our evaluations.
The \ac{ova} technique is employed for multi-class classification~\cite{rifkin2004defense}.
In this approach, \textit{N} binary classifiers are trained for \textit{N} distinct classes.
Each classifier assesses its specific class against all other classes.
The predictions from these binary classifiers are aggregated using a meta-classifier, which integrates their outputs.

In our approach, we utilize a meta-classifier within a machine learning model to enhance the detection of multi-stage cyberattacks. This meta-classifier, an ensemble of various base classifiers, is designed to select the most confident prediction from its constituent classifiers. It employs a windowing technique, analyzing data in segments to identify potential attack patterns. This method flags anomalies based on specific classifications that align with stages of a cyberattack as outlined in the MITRE ATT\&CK Matrix.

Moreover, the softmax function plays a crucial role in this framework. It converts the output of each binary classifier into a probability distribution across different classes, aiding in the decision-making process. This allows for a more nuanced classification approach, rather than a binary decision.

A key aspect of our model is its sequence detection capability, which is particularly adept at recognizing and ordering the stages of multi-stage attacks. This sequence awareness is crucial for identifying attacks that follow or deviate from expected patterns. For example, a typical attack sequence might start with initial access, followed by execution and then persistence, while an atypical sequence could begin in reverse. This sequential logic is being further refined to enhance its efficacy.

Considering the real-time nature of \acp{ids}, a windowing mechanism is introduced to ensure timeliness.
The meta-classifier evaluates a particular time span, ensuring the emergence of a potential multi-stage attack.
It's essential to state that the current scope of our work is confined to scenarios involving a single agent, thus excluding instances of overlapping or concurrent multi-agent attacks.

To shed light on the impact of specific attack parameters on the collective decision, the SHAP framework is leveraged.
This tool aids in ascertaining the contribution of individual features towards the model's prediction for a specific instance~\cite{chen2020true}.
In our architecture, this framework is applied to every base classifier.
In contexts such as multi-stage attacks, mere labeling of events proves inadequate.
However, by explicating each base classifier combined with an intelligible amalgamation methodology, the entirety of the decision-making process becomes comprehensible.
If the fusion technique lacks clarity, the SHAP framework can be redeployed to fathom the influence of each base classifier on the final decision.

The SHAP framework assists in pinpointing the contribution of each feature to the model's decision for any given instance.
This is applied across all base classifiers in our setup.
Mere event labeling becomes inadequate in contexts like multi-stage attacks.
However, by elucidating each base classifier coupled with an interpretable combination method, the entire decision-making process can be understood.
If the combination technique lacks transparency, the SHAP framework can be used again to understand the influence of each base classifier.

An inherent module for the meta-learning was developed, housing the meta-classifier.
The dataset for the study is sourced from ''unified2'' files, which are then parsed to extract pertinent records and transform them into a DataFrame.
The data undergoes preprocessing, where redundant columns are discarded, and categorical data is encoded to integer equivalents.
Labels are then binarized using the ''label-binarize'' function from the ''sklearn.preprocessing'' package, facilitating their use with the meta-classifier.

In our tests, a combination of supervised, unsupervised, and mixed learning techniques is applied to elucidate the contributions of specific features.
Once the data is suitably prepared, the SHAP framework is utilized to depict the influence of distinct attributes on the model's decision.
This interpretation can be visualized using bar plots and beeswarm plots, illustrating the importance of each feature for each class.
The methodology also encompasses a function, which computes the overall impact of each instance based on its SHAP values.

By leveraging a meta-classifier with a windowing technique, our methodology offers a robust mechanism for detecting multi-stage attacks in real-time scenarios.
Furthermore, the SHAP framework provides in-depth insight into feature influence, making the model's decisions more interpretable.
The combination of these techniques and frameworks presents a holistic approach to cybersecurity, ensuring threats are detected with precision and clarity.

The prototype of the process-aware intrusion detection system is designed to vary different information inputs, allowing for an in-depth investigation into how process awareness influences detection quality. This prototype strategically incorporates various data points, such as \ac{it}, \ac{ot}, and \ac{et} attributes, to analyze the impact of diverse information types on identifying cyber threats. By adjusting these inputs and observing the system's response, the study aims to gauge the effectiveness of process-aware approaches in enhancing the accuracy and reliability of intrusion detection in complex environments like smart grids. This methodical experimentation with varied inputs is pivotal in understanding the nuances of process awareness and its role in improving cybersecurity measures.

==> chapter4_old.tex <==
% ############################################################
%           V. RESULTS & DISCUSSION
% ############################################################
\section{Investigation}\label{sec:result}
In this Section we present the investigation findings of our work. In particular, Section~\ref{sec:result_procedure} describes the scenario of the grid as well as the multi-stage cyberattack that is used for the experiments. According to the scenario, we perform the investigation and present the result in Section~\ref{sec:result_findings}, while also discussing them in Section~\ref{sec:result_discussion} in the light of added value of process awareness in intrusion detection.

\subsection{Scenario}\label{sec:result_procedure}
In this study, we have selected the CIGRE grid model as our scenario for a distribution grid, deliberately chosen to exemplify a network with integrated decentralized power generation~\cite{pandapowerCigre}. The accompanying process network assumes all stations are under remote monitoring and control, constituting an \ac{ot} communication infrastructure with routers, switches, firewalls, \ac{scada} systems, and \acp{rtu}. These elements are strategically interconnected and tied to the energy network's operation, ensuring meticulous control and supervision compliant with \ac{iec104} standards, thus facilitating the simulation of power flow and communication within a smart grid framework.

To ensure a comprehensive system analysis, our multi-stage cyberattack integrates several MITRE ATT\&CK recommended techniques in a timely and linear sequence. The initial phase involves \ac{arp} spoofing between two \acp{rtu} and one \ac{mtu}, followed by the establishment of a \ac{mitm} link to forward packets through netfilterqueue. This setup allows complete access to routed packets, enabling their alteration, dropping, or injection. It's crucial to update IP size, \ac{tcp} size, and checksums for accurate packet manipulation.

As the simulation progresses, specific attack strategies are deployed at different intervals. For example, during the initial 10\% of the simulation, \ac{tcp} RST flags are set on packets from the \ac{mtu}, which is recognized as an anomaly in user behavior. Subsequently, between 20\% and 80\% of the simulation, a choice is made between modifying \ac{iec104} cause of transmission and information object values. The latter involves setting incoming \ac{rtu} values to static ones.

In the final stage, between 80\% and 100\% of the simulation, an SSH brute-force attack is executed, targeting an \ac{rtu} not spoofed via \ac{arp}. The brute-force attempt is limited to avoid triggering alarms in other systems.

Post-attack, an \ac{ids} signature recognition process is executed, based on PCAP files that contain traffic observed from all devices. This process includes matching specific patterns for enhanced accuracy and analyzing new approaches. The \ac{ids} system generates detailed events for each packet, encompassing various data points and attack indicators, and categorizes these events into seven distinct groups based on their relevance to different network layers (\ac{it}, \ac{ot}, \ac{et}, etc.).

Each category undergoes a separate classification process, with data sampling to ensure equal representation of all MITRE ATT\&CK techniques. This structured approach allows for a nuanced analysis of attack detection and system response in a sophisticated cyber-physical environment.

We can also simulate a normal operation scenario where no attack-induced events occur, but natural \ac{ict} failures such as communication link breakups happen.

The Table~\ref{table:field_descriptions} provides a structured overview of various fields used in the analysis and monitoring of \ac{it}, \ac{ot}, and \ac{et} network events. It categorizes each element by its operational significance, ranging from timestamps to specific protocol data such as \ac{iec104} values. This organization facilitates a clear understanding of network events and aids in the efficient processing and interpretation of cybersecurity data.

\begin{table}[ht!]
\centering
\caption{Fields of event describing indicators}
\begin{tabular}{|p{2.5cm}|p{5.5cm}|}
\hline
\textbf{Field Name} & \textbf{Description} \\
\hline
timestamp & Event timestamp \\
categorization & Event categorization \\
priority & Event priority level \\
phase & Phase in MITRE ATT\&CK \\
ttp & Tactics, techniques, procedures \\
id & Unique event identifier \\
src\_mac & Source MAC address \\
dst\_mac & Destination MAC address \\
src\_ip & Source IP address \\
dst\_ip & Destination IP address \\
packet\_length & Length of packet \\
protocol & Communication protocol \\
sport & Source port \\
dport & Destination port \\
window\_size & Communication window size \\
payload\_size & Payload size in packet \\
diff\_seq & Sequence number difference \\
diff\_ack & Acknowledgment number difference \\
flag & Flag information in communication \\
rtt & Packet round-trip time \\
frequency\_general & General event frequency \\
frequency\_proto & Protocol-specific event frequency \\
throughput & Network throughput \\
IEC 104 Data & Various IEC 104 protocol fields \\
\hline
\end{tabular}
\label{table:field_descriptions}
\end{table}




\subsection{Case Studies}\label{sec:result_findings}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{figures/processawaer_ids_result.pdf}
    \caption{Comparison between the \ac{it}-only and process-aware \ac{ids} in various scenarios}
    \label{fig:estimation_plot}
    \vspace{-1em}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{figures/it_10.png}
    \caption{Feature analysis with a focus on \ac{it} layer-specific attributes, representing the \acs{dos} attack}
    \label{fig:classification-it-10}
    \vspace{-1em}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{figures/otet_10.png}
    \caption{Feature analysis focusing on the process layer-specific attributes, specifically illustrating the \ac{dos} attack}
    \label{fig:classification-otet-10}
    \vspace{-1em}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{figures/it_12.png}
    \caption{Feature analysis concentrating on the \ac{it} layer-specific attributes, showcasing the \ac{iec104} manipulation}
    \label{fig:classification-it-12}
    \vspace{-1em}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{figures/otet_12.png}
    \caption{Feature analysis concentrating on the process layer-specific attributes, showcasing the \ac{iec104} manipulation}
    \label{fig:classification-otet-12}
    \vspace{-1em}
\end{figure}

In examining the significance of features in detection, we analyze both \ac{it} and process-focused events. Our focus includes multiple \ac{it} attacks (e.g. \ac{dos}) and \ac{iec104}-based manipulation attacks, to understand the impact of domain-specific knowledge on detection effectiveness. The observation within this investigation offer valuable insights into cyberattack detection across \ac{it}, \ac{ot}, and \ac{et} layers. 

Direct comparison of detection quality between \ac{it}-only and process-aware \ac{ids} reveals notable differences in their performance across scenarios (cf. Figure~\ref{fig:estimation_plot}). While both systems perform similarly in \ac{it}-focused events, process-aware \ac{ids} significantly excels in detecting process-focused events, particularly \ac{iec104} manipulation attacks, more accurately than \ac{it}-focused \ac{ids}.

Figure \ref{fig:classification-otet-10} depicts an attack scenario in the \ac{ot} and \ac{et} layers, highlighting general and SYN \ac{dos} attacks. However, the lack of \ac{it} data renders \ac{dos} attacks undetectable in this setup. Instead, the focus is on \ac{iec104} common object address and information object value details, inadvertently missing the real attack. Priority values are less critical here as they indicate the alert level specified by the MITRE ATT\&CK framework, crucial for real-time \ac{ids}.

Contrastingly, Figure \ref{fig:classification-it-10} presents an \ac{it}-oriented attack, including general and SYN \ac{dos}. The window size's bifurcation suggests simplicity in sent packets and limited recipient response. source ports and destination port features imply consistent host involvement, while ack and seq number variations suggest packet loss and disrupted connections in the \ac{dos} scenario.

Figure \ref{fig:classification-it-12} returns to the \ac{it} level, adding \ac{iec104} manipulations. This demonstrates the inadequacy of window size alone for attack indication, underscoring the necessity for \ac{ot} and \ac{et} specific data.

Lastly, Figure \ref{fig:classification-otet-12} explores an attack across \ac{ot} and \ac{et} layers, focusing on \ac{iec104} manipulation. The impact of \ac{iec104} IO value manipulation on system control is significant, and the recurrence of similar \ac{iec104} \acp{coas} within an attack highlights their importance. The figure also indicates a correlation of \ac{iec104} object address with value changes, often seen in attacks executed via the same spoofed line.

\subsection{Discussion}\label{sec:result_discussion}
The investigation demonstrate the performance of \ac{it}-only and process-aware \ac{ids} across various stages of a multi-stage cyberattack, as outlined by the MITRE ATT\&CK framework. The \ac{it}-focused \ac{ids} showed its capabilities in detecting general and SYN \ac{dos} attacks, with the window size clustering and differences in ack and seq numbers indicating packet loss and disturbed connections. However, this approach lacked efficiency in detecting specific types of attacks such as \ac{iec104} manipulations. In contrast, the process-aware \ac{ids}, which considered \ac{ot} and \ac{et} layers, demonstrated a higher efficacy in identifying attacks like \ac{iec104} information object value manipulation, with significant emphasis on \ac{iec104} common object address and cause of transmission manipulation features. This indicates the importance of including \ac{ot} and \ac{et} specific information for a more comprehensive understanding and detection of complex attacks within the system. The process-aware \ac{ids}'s ability to detect subtle manipulations in control systems highlights its advanced capabilities over traditional \ac{it}-focused \ac{ids}.

Furthermore, the results revealed that incorporating \ac{ot} and \ac{et} attributes into the intrusion detection process significantly enhances detection quality. This improvement is particularly notable in scenarios closely related to the system's process layer, such as value manipulation in replay attack events. The \ac{ids} with process-aware attribution demonstrated superior performance in these instances, as observable by Figure~\ref{fig:estimation_plot} between \ac{it} Only and Process Aware \ac{ids}. The inclusion of \ac{ot} and \ac{et} attributes in the detection mechanism provides a more comprehensive understanding of the system's behavior, allowing for more accurate identification and response to specific types of cyber threats. 
Both systems show equal precision, recall, and F1-score in detecting normal activities and \ac{arp} spoofing attacks, indicating their effectiveness in these scenarios. However, differences emerge in detecting \ac{dos} and Value Manipulation attacks. The Process Aware \ac{ids} outperforms \ac{it} Only in \ac{dos} attack detection, with higher precision but slightly lower recall and F1-score. This suggests that Process Aware \ac{ids} can more accurately identify \ac{dos} attacks but may miss a few instances. In Value Manipulation attack detection, the Process Aware \ac{ids} significantly outperforms \ac{it} Only \ac{ids}, with notably higher precision, recall, and F1-score. This implies that Process Aware \ac{ids} is more effective in accurately identifying and responding to Value Manipulation attacks, making it a superior choice for environments where such attacks are a concern.
\vspace{-1em}


==> chapter5_old.tex <==
% ############################################################
%           CONCLUSION
% ############################################################
\section{Conclusion} \label{sec:conclusion}
With the growing integration of \ac{ict} in power grids, new opportunities arise alongside an expanding threat landscape. To devise effective countermeasures in the domains of prevention, detection, and reaction, a deep understanding of the processes is vital. Particularly for detection measures like IDS, process awareness is a critical area of research in cybersecurity. This paper investigates process awareness in intrusion detection, creating a comprehensive environment that simulates a \ac{sg} incorporating \ac{it}, \ac{ot}, and \ac{et} layers within a co-simulation. Moreover, we developed a prototype machine learning-based \ac{ids} to explore the impact of domain-specific attributes on process indicators. Our multi-stage cyberattack simulations, based on the MITRE ATT\&CK Matrix, targeted various layers of the SG. We observed that process-aware \ac{ids}, compared to \ac{it}-only \ac{ids}, improved detection rates in process-centric cyberattack events. In the \ac{it} layer, for events like \ac{dos} and SSH brute-force, the process-aware \ac{ids} performed similarly or slightly better due to access to domain-specific indicators, enabling more precise differentiation from non-malicious \ac{it}-related events. Future research should focus on further developing benchmark environments to evaluate and test sophisticated \ac{ids} in \ac{sg} contexts, and generating comprehensive datasets from these co-simulation environments to serve as digital twins, mirroring individual infrastructure setups.

==> figures/sankey_generator/sankey-doc-preamble.tex <==
\usepackage[paper=a4paper,vmargin=1.5cm,left=4.5cm,right=3.5cm,marginparwidth=3.5cm]{geometry}
\usepackage[utf8]{inputenc}
\usepackage{cmap}
\usepackage[T1]{fontenc}
\usepackage{lmodern}
\usepackage[final,protrusion=true,expansion=true]{microtype}
\usepackage{xcolor}
\PassOptionsToPackage{final,colorlinks,linkcolor=red!60!orange!85!black}{hyperref}
\usepackage{dtxdescribe}
\usepackage[numbered]{hypdoc}
\usepackage{fancyvrb}
\usepackage[final]{listings}
\usepackage{enumitem}
\usepackage{bookmark}
\usepackage{siunitx}
\usepackage{footnote}
\usepackage{etoc}
\usepackage{accsupp}
\usepackage{tikz}
\usetikzlibrary{positioning,patterns.meta,fit}
\usepackage[british]{babel}
\usepackage{varioref}
\usepackage{embedfile}
\usepackage{dtx-attach}
\embedfile[mimetype=text/plain]{sankey.ins}
\usepackage{sankey}

\colorlet{bgcode}{yellow!50!gray!10}
\colorlet{keyword}{blue!50!cyan!50!black}
\colorlet{comment}{red!75!black}

\newcommand\emptyaccsupp[1]{\BeginAccSupp{ActualText={}}#1\EndAccSupp{}}

\lstset{
  literate=
  {Ã¡}{{\'a}}1 {Ã©}{{\'e}}1 {Ã­}{{\'i}}1 {Ã³}{{\'o}}1 {Ãº}{{\'u}}1
  {Ã}{{\'A}}1 {Ã‰}{{\'E}}1 {Ã}{{\'I}}1 {Ã“}{{\'O}}1 {Ãš}{{\'U}}1
  {Ã }{{\`a}}1 {Ã¨}{{\`e}}1 {Ã¬}{{\`i}}1 {Ã²}{{\`o}}1 {Ã¹}{{\`u}}1
  {Ã€}{{\`A}}1 {Ãˆ}{{\'E}}1 {ÃŒ}{{\`I}}1 {Ã’}{{\`O}}1 {Ã™}{{\`U}}1
  {Ã¤}{{\"a}}1 {Ã«}{{\"e}}1 {Ã¯}{{\"i}}1 {Ã¶}{{\"o}}1 {Ã¼}{{\"u}}1
  {Ã„}{{\"A}}1 {Ã‹}{{\"E}}1 {Ã}{{\"I}}1 {Ã–}{{\"O}}1 {Ãœ}{{\"U}}1
  {Ã¢}{{\^a}}1 {Ãª}{{\^e}}1 {Ã®}{{\^i}}1 {Ã´}{{\^o}}1 {Ã»}{{\^u}}1
  {Ã‚}{{\^A}}1 {ÃŠ}{{\^E}}1 {ÃŽ}{{\^I}}1 {Ã”}{{\^O}}1 {Ã›}{{\^U}}1
  {Å“}{{\oe}}1 {Å’}{{\OE}}1 {Ã¦}{{\ae}}1 {Ã†}{{\AE}}1 {ÃŸ}{{\ss}}1
  {Ã§}{{\c c}}1 {Ã‡}{{\c C}}1 {Ã¸}{{\o}}1 {Ã¥}{{\r a}}1 {Ã…}{{\r A}}1
  {â‚¬}{{\texteuro}}1 {Â£}{{\pounds}}1 {Â°}{{\degres}}1
  {â€™}{{\textquoteright}}1 {â€˜}{{\textquoteleft}}1
  {Â«}{{<<}}1 {Â»}{{>>}}1
  {â€”}{{---}}1 {âˆ’}{{$-$}}1
  {\^\^A}{{}}0                % verbatim in .dtx file
}

\lstset{
  fancyvrb=true,
  escapechar=`,
  extendedchars=true,
  fontadjust=true,
  columns=fullflexible,
  flexiblecolumns=true,
  inputencoding=utf8,
  keepspaces=true,
  backgroundcolor=\color{bgcode},
  basicstyle=\mdseries\ttfamily,
  keywordstyle=\color{keyword},
  stringstyle=\ttfamily\color{green!50!black},
  commentstyle=\color{comment}\itshape,
  emphstyle=\bfseries\color{red},
  numbersep=5pt,
  %numbers=left,
  numberstyle=\tiny\emptyaccsupp,
  showstringspaces=false,
  upquote=true,
  aboveskip=.5\parskip,
  belowskip=.5\parskip,
  framexleftmargin=1pt,
  framexrightmargin=1pt,
  gobble=2,              % \lstlisting code in .dtx
}

\lstdefinestyle{textsmall}{basicstyle=\color{black}\small\mdseries\ttfamily}
\lstdefinestyle{textfootnotesize}{basicstyle=\color{black}\footnotesize\mdseries\ttfamily}
\lstdefinestyle{textscriptsize}{basicstyle=\color{black}\scriptsize\mdseries\ttfamily}
\lstdefinestyle{texttiny}{basicstyle=\color{black}\tiny\mdseries\ttfamily}

\lstdefinestyle{bash}{
  language=bash,
  backgroundcolor=\color{gray!10},
}
\lstdefinestyle{bashsmall}{style=bash,style=textsmall}
\lstdefinestyle{bashfootnotesize}{style=bash,style=footnotesize}
\lstdefinestyle{bashscriptsize}{style=bash,style=scriptsize}

\lstdefinestyle{LaTeX}{
  language=[LaTeX]TeX,
  moretexcs={
    Lab,
    LabSet,
    Qty,
    QtySet,
    colorlet,
    coordinate,
    countries,
    country,
    countryname,
    definecolor,
    draw,
    endcountry,
    fill,
    foreach,
    hashband,
    hdist,
    hwidth,
    node,
    nodename,
    path,
    sankeyadvance,
    sankeydubins,
    sankeyend,
    sankeyend,
    sankeyfork,
    sankeynode,
    sankeynodealias,
    sankeynodeend,
    sankeynodestart,
    sankeyoutin,
    sankeyset,
    sankeystart,
    sankeyturn,
    sankeyturnleft,
    sankeyturnleftbackward,
    sankeyturnright,
    sankeyturnrightbackward,
    sisetup,
    startcountry,
    tikzset,
    turnandstop,
    usepackage,
    vdist,
  }
}
\lstdefinestyle{LaTeXsmall}{style=LaTeX,style=textsmall}
\lstdefinestyle{LaTeXfootnotesize}{style=LaTeX,style=textfootnotesize}
\lstdefinestyle{LaTeXscriptsize}{style=LaTeX,style=textscriptsize}
\lstdefinestyle{LaTeXtiny}{style=LaTeX,style=texttiny}

\def\code{\lstinline[basicstyle=\mdseries\ttfamily\color{red!50!black}]}

\edef\samplecodename{\jobname-code.vrb}

\newcommand\constant[1]{\textcolor{violet}{\texttt{#1}}}
\newcommand\ARG[1]{\texttt{\{#1\}}}
\newcommand\OPTARG[1]{\textcolor{green!50!black}{\texttt{[#1]}}}
\newcommand\VAR[1]{\textit{\texttt{\ensuremath{\langle}#1\ensuremath{\rangle}}}}
\newcommand\NOTE[1]{\leavevmode\marginpar{#1}}

\def\mynobreakpar{\par\nobreak\@afterheading}
\def\docprefix#1{\texttt{\textcolor{gray}{#1}}}
\def\sankeykeysprefix{/sankey}

\newenvironment{sankeyoption}[5][]{% [prefix] key, val, default, initially
  \begingroup
  %
  \def\keypath{#1}%
  \ifdefempty{\keypath}{\def\keypath{\sankeykeysprefix}}{}%
  \def\key{#2}%
  \def\val{#3}%
  \def\default{#4}%
  \def\initially{#5}%
  %\setlength\parindent{\dimexpr.5\parindent\relax}%
  % \vspace{.25\baselineskip plus .25\baselineskip minus 0mm}
  \parfillskip 0pt plus 1fil%
  \leavevmode%
  \DescribeKey{\key}%
  \ttfamily%
  %\hspace*{-1cm}%
  \textcolor{red!75!black}{\texttt{\docprefix{\keypath/}\key}}%
  \ifdefempty{\val}{}{=\val}%
  \hfill%
  \ifdefempty{\default}{\null}{(default:\,\constant{\default})}%
  \ifdefempty{\initially}{\null}{(initially:\,\constant{\initially})}%
  \mynobreakpar%
  \endgroup%
  \parskip=.5\baselineskip plus .25\baselineskip minus .25\baselineskip
  \parfillskip=30pt plus 1fil
  \itemize[topsep=0pt,partopsep=0pt,itemsep=0pt]\item[]
}{%
  \enditemize%
}

\newcommand\MACRO{\hspace*{0cm}}

\newlist{sankeyconstantsdesc}{description}{1}
\setlist[sankeyconstantsdesc]{align=right,labelindent=1.5em,labelsep=.5em,leftmargin=!,font=\normalfont}

\newlength{\myparskip}
\setlength{\myparskip}{.75\baselineskip plus 8\baselineskip minus .25\baselineskip}
\usepackage[skip=\myparskip]{parskip}
\newenvironment{miniblock}{%
  \vspace{.5\parskip}%
}{%
}

\tikzset{
  every picture/.style={
    execute at end picture={
      \begin{pgfonlayer}{background}
        \node[fit=(current bounding box),inner sep=0](bb){};
        \def\rs{5mm}
        \draw[gray!25] let
        \p{sw}=(bb.south west), \p{ne}=(bb.north east),
        \n{maxx}={ceil(\x{ne}/\rs)*\rs}, \n{minx}={floor(\x{sw}/\rs)*\rs},
        \n{maxy}={ceil(\y{ne}/\rs)*\rs}, \n{miny}={floor(\y{sw}/\rs)*\rs}
        in (\n{minx},\n{miny}) grid (\n{maxx},\n{maxy});
        \begin{scope}[overlay]
          \draw[gray!50,-latex] let
          \p{sw}=(bb.south west), \p{ne}=(bb.north east),
          \n{maxx}={ceil(\x{ne}/\rs)*\rs}, \n{minx}={floor(\x{sw}/\rs)*\rs},
          \n{maxy}={ceil(\y{ne}/\rs)*\rs}, \n{miny}={floor(\y{sw}/\rs)*\rs}
          in (\n{minx},0) -- (\n{maxx}+1mm,0);
          \draw[gray!50,-latex] let
          \p{sw}=(bb.south west), \p{ne}=(bb.north east),
          \n{maxx}={ceil(\x{ne}/\rs)*\rs}, \n{minx}={floor(\x{sw}/\rs)*\rs},
          \n{maxy}={ceil(\y{ne}/\rs)*\rs}, \n{miny}={floor(\y{sw}/\rs)*\rs}
          in (0,\n{miny}) -- (0,\n{maxy}+1mm);
        \end{scope}
      \end{pgfonlayer}
    }
  }
}

\def\MacroFont{
  \fontencoding\encodingdefault
  \fontfamily\ttdefault
  \fontseries\mddefault
  \fontshape\updefault
  \footnotesize
}

\renewcommand*{\DescribeMacro}[2][]{%
  \@bsphack%
  \@ifundefined{@captype}{% not float?
    \leavevmode%
    \marginpar{%
      \hbadness=10000%
      \hfuzz=5em%
      \raggedleft%
      \ifblank{#1}{}{{\scriptsize\textsf{[#1]}} }% class
      \MacroFont\cmd{#2}% name
    }% marginpar
  }{}% not float?
  \begingroup%
  \DTXD@origwrindex{%
    \DTXD@macroname{#2}\actualchar\DTXD@verbatimcmd{#2}% name
    \ifblank{#1}{}{\levelchar[#1]}% class
    \encapchar usage}%
  \ifblank{#1}%
  {}% no class
  {% class given
    \begingroup%
    \DTXD@origwrindex{%
      #1\actualchar[#1]:\levelchar%
      \DTXD@macroname{#2}\actualchar\DTXD@verbatimcmd{#2}%
      \encapchar usage}%
  }% class given
  \@esphack%
  \ignorespaces%
}


==> figures/sankey_generator/tikzlibrarydubins.code.tex <==
%%
%% This is file `tikzlibrarydubins.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% sankey.dtx  (with options: `tikzlibrarydubins.code.tex')
%% 
%% This is a generated file.
%% 
%% Copyright (C) 2016, 2021 by Paul Gaborit
%% 
%% This work may be distributed and/or modified under the conditions of the
%% LaTeX Project Public License, either version 1.3 of this license or (at
%% your option) any later version.  The latest version of this license is
%% in
%% 
%% <http://www.latex-project.org/lppl.txt>
%% 
%% and version 1.3 or later is part of all distributions of LaTeX version
%% 2005/12/01 or later.
%% 
%% This work has the LPPL maintenance status “maintained”.
%% 
%% The Current Maintainer of this work is Paul Gaborit.
%% 
%% This work consists of the files sankey.dtx, sankey.ins and the derived
%% files sankey.sty, tikzlibrarydubins.code.tex, sankey-doc-preamble.sty,
%% sankey-example1.tex, sankey-example2.tex, sankey-example3.tex,
%% sankey-example3-variation.tex, sankey-example4.tex,
%% sankey-example-energy.tex
%% 
\def\tikzlibrarydubins@version{v3.0.1}
\def\tikzlibrarydubins@date{2022/02/04}
\usetikzlibrary{calc}
\RequirePackage{etoolbox}
\RequirePackage{xfp}

\newbool{dubinspathreverse}
\def\ifpgfmathcond#1{%
  \pgfmathparse{(#1)?1:0}%
  \ifnumequal{\pgfmathresult}{1}%
}
\def\dbp@getxy#1#2#3{%
  \tikz@scan@one@point\pgfutil@firstofone(#3)\relax%
  \edef#1{\the\pgf@x}%
  \edef#2{\the\pgf@y}%
}
\def\dbp@anglebetween#1#2#3{%macro, s, t
  \dbp@getxy\dbp@ax\dbp@ay{#2}
  \dbp@getxy\dbp@bx\dbp@by{#3}
  \pgfmathsetmacro#1{atan2(\dbp@by-\dbp@ay,\dbp@bx-\dbp@ax)}
}
\def\dbp@distancebetween#1#2#3{%macro, s, t
  \dbp@getxy\dbp@ax\dbp@ay{#2}
  \dbp@getxy\dbp@bx\dbp@by{#3}
  \edef#1{\fpeval{sqrt(%
      (\dbp@bx-\dbp@ax)*(\dbp@bx-\dbp@ax)%
      +(\dbp@by-\dbp@ay)*(\dbp@by-\dbp@ay)%
      )}}%
}
\newcommand\dbp@rsr{% s, sa, t, ta, as, len, at, r
  let
  \p{tr}=([shift={(\dbp@angb-90:\dbp@radius pt)}]\dbp@b),
  \n1={\dbp@anga+90},
  \n2={\dbp@angb+90},
  \n3={\n2+\dbp@lastangle}
  in
  arc(\n1:\n1-\dbp@firstangle:\dbp@rradius pt)
  -- ([shift={(\p{tr})}]\n3:\dbp@rradius pt)
  arc(\n3:\n2:\dbp@rradius pt)
}
\newcommand\dbp@lsl{% s, sa, t, ta, as, len, at, r
  let
  \p{tl}=([shift={(\dbp@angb+90:\dbp@radius pt)}]\dbp@b),
  \n1={\dbp@anga-90},\n2={\n1+\dbp@firstangle},
  \n3={\dbp@angb-90},\n4={\n3-\dbp@lastangle}
  in
  arc(\n1:\n2:\dbp@lradius pt)
  -- ([shift={(\p{tl})}]\n4:\dbp@lradius pt)
  arc(\n4:\n3:\dbp@lradius pt)
}
\newcommand\dbp@rsl{% s, sa, t, ta, as, len, at, r
  let
  \p{tl}=([shift={(\dbp@angb+90:\dbp@radius pt)}]\dbp@b),
  \n1={\dbp@anga+90},\n2={\n1-\dbp@firstangle},
  \n3={\dbp@angb-90},\n4={\n3-\dbp@lastangle}
  in
  arc(\n1:\n2:\dbp@rradius pt)
  -- ([shift={(\p{tl})}]\n4:\dbp@lradius pt)
  arc(\n4:\n3:\dbp@lradius pt)
}
\newcommand\dbp@lsr{% s, sa, t, ta, as, len, at, r
  let
  \p{tr}=([shift={(\dbp@angb-90:\dbp@radius pt)}]\dbp@b),
  \n1={\dbp@anga-90},\n2={\n1+\dbp@firstangle},
  \n3={\dbp@angb+90},\n4={\n3+\dbp@lastangle}
  in
  arc(\n1:\n2:\dbp@lradius pt)
  -- ([shift={(\p{tr})}]\n4:\dbp@rradius pt)
  arc(\n4:\n3:\dbp@rradius pt)
}
\newcommand\dbp@lrl{% s, sa, t, ta, as, ai, at, r
  let
  \n1={\dbp@anga-90},\n2={\n1+\dbp@firstangle},
  \n3={\dbp@angb-90},\n4={\n3-\dbp@lastangle}
  in
  arc(\n1:\n2:\dbp@lradius pt)
  arc(\n2+180:\n2+180-\dbp@midparam:\dbp@rradius pt)
  arc(\n4:\n3:\dbp@lradius pt)
}
\newcommand\dbp@rlr{% s, sa, t, ta, as, ai, at, r
  let
  \n1={\dbp@anga+90},\n2={\n1-\dbp@firstangle},
  \n3={\dbp@angb+90},\n4={\n3+\dbp@lastangle}
  in
  arc(\n1:\n2:\dbp@rradius pt)
  arc(\n2+180:\n2+180+\dbp@midparam:\dbp@lradius pt)
  arc(\n4:\n3:\dbp@rradius pt)
}
\newcommand\dbp@rev@lsl{\dbp@rsr}
\newcommand\dbp@rev@rsr{\dbp@lsl}
\newcommand\dbp@rev@lsr{\dbp@lsr}
\newcommand\dbp@rev@rsl{\dbp@rsl}
\newcommand\dbp@rev@lrl{\dbp@rlr}
\newcommand\dbp@rev@rlr{\dbp@lrl}
\newcommand\dubinspath[1]{%
  \pgfextra{
    \dubinspathset{#1}
    \ifbool{dubinspathreverse}{
      \edef\dbp@newa{\dbp@b}
      \edef\dbp@newb{\dbp@a}
      \pgfmathsetmacro\dbp@newanga{180+\dbp@angb}
      \pgfmathsetmacro\dbp@newangb{180+\dbp@anga}
      \edef\dbp@newfirstangle{\dbp@lastangle}
      \edef\dbp@newlastangle{\dbp@firstangle}
      \edef\dbp@newmethod{rev@\dbp@method}
      \edef\dbp@newlradius{\dbp@rradius}
      \edef\dbp@newrradius{\dbp@lradius}
      \dubinspathset{
        start point=\dbp@newa,
        end point=\dbp@newb,
        start angle=\dbp@newanga,
        end angle=\dbp@newangb,
        first angle=\dbp@newfirstangle,
        last angle=\dbp@newlastangle,
        left and right minimum radii=\dbp@newlradius pt and \dbp@newrradius pt,
        method=\dbp@newmethod,
      }
    }{}
  }
  \csname dbp@\dbp@method\endcsname%
}
\def\dbp@store#1#2{%
  \expandafter\xdef\csname dbp@store@#1@#2\endcsname%
  {\csname dbp@#2\endcsname}%
}
\def\dbp@get#1#2{%
  \csname dbp@store@#1@#2\endcsname%
}
\def\dbp@setparams#1#2#3#4#5{%
  % method, length, fisrt angle, middle param, last angle
  \edef\dbp@method{#1}
  \edef\dbp@length{#2}
  \edef\dbp@firstangle{#3}
  \edef\dbp@middleparam{#4}
  \edef\dbp@lastangle{#5}
  \ifdef{\dbp@storename}{
    \foreach \p in {method,length,firstangle,middleparam,lastangle}{
      \dbp@store{\dbp@storename}{\p}
    }
  }{}
}
\def\dbp@updateparams#1#2#3#4#5{
  \ifpgfmathcond{#2<\dbp@length}{
    \dbp@setparams{#1}{#2}{#3}{#4}{#5}
  }{}
}
\tikzset{
  dubins path/.is family,
  dubins path,
  start point/.store in=\dbp@a,
  start angle/.store in=\dbp@anga,
  end point/.store in=\dbp@b,
  end angle/.store in=\dbp@angb,
  store/.store in=\dbp@storename,
  use store/.style={
    method=\dbp@get{#1}{method},
    first angle=\dbp@get{#1}{firstangle},
    last angle=\dbp@get{#1}{lastangle},
    middle param=\dbp@get{#1}{middleparam},
  },
  minimum radius/.code={
    \pgfmathsetmacro\dbp@radius{#1}
    \pgfmathsetmacro\dbp@rradius{#1}
    \pgfmathsetmacro\dbp@lradius{#1}
  },
  left and right minimum radii/.code args={#1 and #2}{
    \pgfmathsetmacro\dbp@lradius{#1}
    \pgfmathsetmacro\dbp@rradius{#2}
    \pgfmathsetmacro\dbp@radius{(\dbp@lradius + \dbp@rradius)/2}
  },
  method/.store in=\dbp@method,
  first angle/.store in=\dbp@firstangle,
  last angle/.store in=\dbp@lastangle,
  middle param/.store in=\dbp@midparam,
  reverse/.is if=dubinspathreverse,
}
\newcommand\dubinspathset[1]{\tikzset{dubins path,#1}}
\newcommand\dubinspathcalc[1]{%
  \begingroup
  \dubinspathset{#1}
  \tikzset{
    declare function={
      angtodist(\dbp@a,\dbp@r)={abs(\dbp@a)*.01745329*\dbp@r};
      modangr(\dbp@a,\dbp@b)={
        (
        Mod(\dbp@a,360)<Mod(\dbp@b,360)
        ?
        Mod(\dbp@a,360)
        :
        Mod(\dbp@a,360)-360)+\dbp@b-Mod(\dbp@b,360
        )
      };
      modangl(\dbp@a,\dbp@b)={
        (
        Mod(\dbp@a,360)<Mod(\dbp@b,360)
        ?
        Mod(\dbp@a,360)+360
        :
        Mod(\dbp@a,360))+(\dbp@b)-Mod(\dbp@b,360)
      };
    },
  }

  \pgfmathsetmacro\dbp@radius{\dbp@rradius}
  \pgfmathsetmacro\dbp@anga{mod((\dbp@anga)+180,360)-180}
  \pgfmathsetmacro\dbp@angb{mod((\dbp@angb)+180,360)-180}
  \path
  let
  \p{a}=(\dbp@a),
  \p{b}=(\dbp@b),
  \p{ar}=($(\p{a}) + (\dbp@anga-90:\dbp@radius pt)$),
  \p{al}=($(\p{a}) + (\dbp@anga+90:\dbp@radius pt)$),
  \p{br}=($(\p{b}) + (\dbp@angb-90:\dbp@radius pt)$),
  \p{bl}=($(\p{b}) + (\dbp@angb+90:\dbp@radius pt)$)
  in \pgfextra{
    \pgfinterruptpath

    % RSR (ar and br)
    \dbp@anglebetween\dbp@rsrarbr{\p{ar}}{\p{br}}
    \dbp@distancebetween\dbp@rsrdarbr{\p{ar}}{\p{br}}
    \pgfmathsetmacro\dbp@rsrangone{Mod(\dbp@anga-\dbp@rsrarbr,360)}
    \pgfmathsetmacro\dbp@rsrangtwo{Mod(\dbp@rsrarbr-\dbp@angb,360)}
    \pgfmathsetmacro\dbp@rsrlen{\dbp@rsrdarbr}
    \pgfmathsetmacro\dbp@rsrdist{
      angtodist(\dbp@rsrangone,\dbp@radius)
      +\dbp@rsrlen
      +angtodist(\dbp@rsrangtwo,\dbp@radius)
    }
    \dbp@setparams{rsr}{\dbp@rsrdist}{\dbp@rsrangone}{\dbp@rsrlen}{\dbp@rsrangtwo}

    % LSL (al and bl)
    \dbp@anglebetween\dbp@lslalbl{\p{al}}{\p{bl}}
    \dbp@distancebetween\dbp@lsldalbl{\p{al}}{\p{bl}}
    \pgfmathsetmacro{\dbp@lslangone}{mod(\dbp@lslalbl-\dbp@anga+720,360)}
    \pgfmathsetmacro{\dbp@lslangtwo}{mod(\dbp@angb-\dbp@lslalbl+720,360)}
    \pgfmathsetmacro\dbp@lsllen{\dbp@lsldalbl}
    \pgfmathsetmacro\dbp@lsldist{
      angtodist(\dbp@lslangone,\dbp@radius)
      +\dbp@lsllen
      +angtodist(\dbp@lslangtwo,\dbp@radius)
    }
    \dbp@updateparams%
    {lsl}{\dbp@lsldist}{\dbp@lslangone}{\dbp@lsllen}{\dbp@lslangtwo}

    % RSL (ar and bl)
    \dbp@distancebetween\dbp@rsldarbl{\p{ar}}{\p{bl}}
    \pgfmathtruncatemacro\dbp@rslok{(\dbp@rsldarbl>=2*\dbp@radius)?1:0}
    \ifnumequal{\dbp@rslok}{1}{
      \dbp@anglebetween\dbp@rslarbl{\p{ar}}{\p{bl}}
      \pgfmathsetmacro\dbp@rslanglesup{
        asin(\dbp@radius/\dbp@rsldarbl*2)}
      \pgfmathsetmacro\dbp@rslangone
      {Mod(\dbp@anga-\dbp@rslarbl+\dbp@rslanglesup,360)}
      \pgfmathsetmacro\dbp@rslangtwo
      {Mod(\dbp@angb-\dbp@rslarbl+\dbp@rslanglesup,360)}
      \pgfmathsetmacro\dbp@rsllen{veclen(\dbp@rsldarbl,\dbp@radius)}
      \pgfmathsetmacro\dbp@rsldist{
        angtodist(\dbp@rslangone,\dbp@radius)
        +\dbp@rsllen
        +angtodist(\dbp@rslangtwo,\dbp@radius)
      }

      \dbp@updateparams%
      {rsl}{\dbp@rsldist}{\dbp@rslangone}{\dbp@rsllen}{\dbp@rslangtwo}
    }{}

    % LSR (al and br)
    \dbp@distancebetween\dbp@lsrdalbr{\p{al}}{\p{br}}
    \pgfmathtruncatemacro\dbp@lsrok{(\dbp@lsrdalbr>=2*\dbp@radius)?1:0}
    \ifnumequal{\dbp@lsrok}{1}{
      \dbp@anglebetween\dbp@lsralbr{\p{al}}{\p{br}}
      \pgfmathsetmacro\dbp@lsranglesup{
        asin(\dbp@radius/\dbp@lsrdalbr*2)}
      \pgfmathsetmacro\dbp@lsrangone
      {Mod(\dbp@lsralbr+\dbp@lsranglesup-\dbp@anga,360)}
      \pgfmathsetmacro\dbp@lsrangtwo
      {Mod(\dbp@lsralbr+\dbp@lsranglesup-\dbp@angb,360)}
      \pgfmathsetmacro\dbp@lsrlen{veclen(\dbp@lsrdalbr,\dbp@radius)}
      \pgfmathsetmacro\dbp@lsrdist{
        angtodist(\dbp@lsrangone,\dbp@radius)
        +\dbp@lsrlen
        +angtodist(\dbp@lsrangtwo,\dbp@radius)
      }
      \dbp@updateparams%
      {lsr}{\dbp@lsrdist}{\dbp@lsrangone}{\dbp@lsrlen}{\dbp@lsrangtwo}
    }{}

    % LRL (al and bl)
    \dbp@distancebetween\dbp@lrldalbl{\p{al}}{\p{bl}}
    \pgfmathtruncatemacro\dbp@lrlok{(\dbp@lrldalbl<=4*\dbp@radius)?1:0}
    \ifnumequal{\dbp@lrlok}{1}{
      \dbp@anglebetween\dbp@lrlalbl{\p{al}}{\p{bl}}
      \pgfmathsetmacro\dbp@lrlangsup{acos(\dbp@lrldalbl/\dbp@radius/4)}
      \pgfmathsetmacro\dbp@lrlangone{
        modangl(\dbp@lrlalbl+\dbp@lrlangsup,\dbp@anga-90)-(\dbp@anga-90)}
      \pgfmathsetmacro\dbp@lrlangtwo{%
        (\dbp@angb-90)-modangr(\dbp@lrlalbl+180-\dbp@lrlangsup,\dbp@angb-90)}
      \pgfmathsetmacro\dbp@lrlangthree{360-2*(90-\dbp@lrlangsup)}
      \pgfmathsetmacro\dbp@lrldist{
        angtodist(\dbp@lrlangone,\dbp@radius)
        +angtodist(\dbp@lrlangthree,\dbp@radius)
        +angtodist(\dbp@lrlangtwo,\dbp@radius)
      }
      \dbp@updateparams%
      {lrl}{\dbp@lrldist}{\dbp@lrlangone}{\dbp@lrlangthree}{\dbp@lrlangtwo}
    }{}

    % RLR (ar and br)
    \dbp@distancebetween\dbp@rlrdarbr{\p{ar}}{\p{br}}
    \pgfmathtruncatemacro\dbp@rlrok{(\dbp@rlrdarbr<=4*\dbp@radius)?1:0}
    \ifnumequal{\dbp@rlrok}{1}{
      \dbp@anglebetween\dbp@rlrarbr{\p{ar}}{\p{br}}
      \pgfmathsetmacro\dbp@rlrangsup{acos(\dbp@rlrdarbr/\dbp@radius/4)}
      \pgfmathsetmacro\dbp@rlrangone{
        (\dbp@anga+90)-modangr(\dbp@rlrarbr-\dbp@rlrangsup,\dbp@anga+90)}
      \pgfmathsetmacro\dbp@rlrangtwo{%
        modangl(\dbp@rlrarbr+180+\dbp@rlrangsup,\dbp@angb+90)-(\dbp@angb+90)}
      \pgfmathsetmacro\dbp@rlrangthree{360-2*(90-\dbp@rlrangsup)}
      \pgfmathsetmacro\dbp@rlrdist{
        angtodist(\dbp@rlrangone,\dbp@radius)
        +angtodist(\dbp@rlrangthree,\dbp@radius)
        +angtodist(\dbp@rlrangtwo,\dbp@radius)
      }
      \dbp@updateparams%
      {rlr}{\dbp@rlrdist}{\dbp@rlrangone}{\dbp@rlrangthree}{\dbp@rlrangtwo}
    }{}

    \endpgfinterruptpath
  };
  \endgroup
}
\endinput
%%
%% End of file `tikzlibrarydubins.code.tex'.

